On the Bursty Evolution of Online Social Networks

The high level of dynamics in today's online social networks (OSNs) creates new challenges for their infrastructures and providers. In particular, dynamics involving edge creation has direct implications on strategies for resource allocation, data partitioning and replication. Understanding network dynamics in the context of physical time is a critical first step towards a predictive approach towards infrastructure management in OSNs. Despite increasing efforts to study social network dynamics, current analyses mainly focus on change over time of static metrics computed on snapshots of social graphs. The limited prior work models network dynamics with respect to a logical clock. In this paper, we present results of analyzing a large timestamped dataset describing the initial growth and evolution of Renren, the leading social network in China. We analyze and model the burstiness of link creation process, using the second derivative, i.e. the acceleration of the degree. This allows us to detect bursts, and to characterize the social activity of a OSN user as one of four phases: acceleration at the beginning of an activity burst, where link creation rate is increasing; deceleration when burst is ending and link creation process is slowing; cruising, when node activity is in a steady state, and complete inactivity.

==> section3.tex <==
\section{Dataset}
The main obstacle to studying dynamics is the difficulty of obtaining detailed data describing OSN dynamics. In this study we got access to an anonymized dataset that contains the timestamped creation of all users and edges in the Renren network.
Renren is the largest online social network in China. Similarly to Facebook, Renren was originally designed for college students. Renren was original named Xiaonei (i.e., in school), then when it started to incorporate other smaller local OSN attempts and allow non university students it officially became RenRen (i.e. everyone).

We host an anonymized dataset that describes the evolution of each nodes as stamped edges in the network. 
The first edge created in the entire Renren history dates back to November 22, 2005 and we host the complete evolution of the first 60000 nodes for a total of 8 millions timed edges events. In total our dataset covers a period of one year from November '05 to December '06.
